Group Properties of Polar Codes for Automorphism Ensemble Decoding

In this paper, we propose an analysis of the automorphism group of polar codes, with the scope of designing codes tailored for automorphism ensemble (AE) decoding. We prove the equivalence between the notion of decreasing monomial codes and the universal partial order (UPO) framework for the description of polar codes. Then, we analyze the algebraic properties of the affine automorphisms group of polar codes, providing a novel description of its structure and proposing a classification of automorphisms providing the same results under permutation decoding. Finally, we propose a method to list all the automorphisms that may lead to different candidates under AE decoding; by introducing the concept of redundant automorphisms, we find the maximum number of permutations providing possibly different codeword candidates under AE-SC, proposing a method to list all of them. A numerical analysis of the error correction performance of AE algorithm for the decoding of polar codes concludes the paper.

==> EC_identification.tex <==
In previous section we have seen that $\EC$ search can be decomposed into the search of cosets of $\GL(s_i) / \BLTA(s_{i,1},\ldots,s_{i,j_i})$. 
Here we focus on these cosets, and we use the PUL matrix decomposition to further simplify the representatives search. 
\begin{definition}[PUL decomposition]
	The permutations $P \in \PL$, $U \in \UTL$ and $(L,b_0) \in \LTA$ are called the PUL decomposition of $(A,b)$ if
	\begin{equation*}
		A v + b = P \cdot U \cdot (L v + b_0 ) ,
	\end{equation*}
	i.e., if $A = P U L$ and $b = P U b_0$.
\end{definition}

\begin{lemma}
	The PUL decomposition exists for all $A \in \GA$ and is not necessarily unique.
\end{lemma}
\begin{proof}
	The existence of the LU decomposition and its non-uniqueness are well known for matrices, and the PUL decomposition is merely a variation thereof, cf.\ Section~\ref{sec:PUL}.
\end{proof}

Note that the PUL decomposition of $(A,b)$ corresponds to the concatenation of the permutations as
\begin{equation}
	\pi_{(A,b)} = \pi_{L,b_0} \circ \pi_U \circ \pi_P  ,
\end{equation}
applied from right to left. %, according to Lemma~\ref{lem:GL-concat}.
By Lemma~\ref{lem:LTA_SC}, we have that under SC decoding $\pi_{L,b_0} \in [\pid]$
As a consequence, cosets of $\EC_i$ can be decomposed as the product of two automorphisms, one belonging to $\mathcal{U}$ and the other belonging to $\mathcal{P}$. 

If we call $\mathcal{A}_{\mathcal{P}}$ and $\mathcal{A}_{\mathcal{U}}$, the subgroups of $\mathcal{A}$ containing only PL and UTL automorphisms, we can always find an EC representative composing elements from these two sets. 
%Figure~\ref{fig:BLTA_EC} shows an example of pattern $A=PU$ with $P\in\mathcal{A}_{\mathcal{P}}$ and $ U\in\mathcal{A}_{\mathcal{U}}$.
\begin{lemma}\label{lem:PU_BLT}
Each EC contains at least one automorphism $P \cdot U$ with $P\in\mathcal{A}_{\mathcal{P}}$ and $U\in\mathcal{A}_{\mathcal{U}}$.
\begin{proof}
Given a representative $A$ for an equivalence class, it is possible to decompose this matrix as $A = P U L$. 
Since $L \in \LTA \leq [\pid]$, then $L^{-1} \in [\pid]$ and hence $A \cdot L^{-1} = PU$ belongs to the same EC as $A$, i.e., $[PU] = [A]$.
\end{proof}
\end{lemma}
For a block structure $S=(s_1,\dots,s_t)$, the number of UTL and PL automorphisms are:
%\begin{align}\label{eq:aut_U}
%	|\mathcal{A}_{\mathcal{U}}| &= \prod_{i=1}^{t}2^{\frac{s_i(s_i-1)}{2}}\\
%	|\mathcal{A}_{\mathcal{P}}| &= \prod_{i=1}^{t}(s_i!)~.\label{eq:aut_P}
%\end{align}
\begin{equation}\label{eq:aut_U_P}
	|\mathcal{A}_{\mathcal{U}}| = \prod_{i=1}^{t}2^{\frac{s_i(s_i-1)}{2}} \quad , \quad |\mathcal{A}_{\mathcal{P}}| = \prod_{i=1}^{t}(s_i!)~.
\end{equation}
%Our heuristic selection is based on a pair of Hamming distances thresholds $D=(d_{U},d_{P})$, representing the minimum distances between two EC representatives in the $M$ automorphisms selected for AE decoding. 
%Every new EC representative is constructed by randomly generating two vectors $v$ and $p$, respectively representing a matrix in $\mathcal{A}_\mathcal{U}$ and $\mathcal{A}_\mathcal{P}$, and checking if the distances between the generated vectors and the vectors already in the EC representative lists are above the thresholds. 
A further check is required to assure that the EC representative does not belong to an already calculated EC. 
This check is done by multiplying the calculated $UP$ matrix and the $UP$ matrices of the previously calculated ECs as stated in Lemma~\ref{lem:checkproductA}. 
%either using $[\pid]=\LTL$ for polar code with block structure $S=(s_0=1,\dots,s_l)$, $[\pid]=\BLTL(2,1,\dots,1)$ otherwise.
\begin{lemma}\label{lem:checkproductA}
Given $\pi_1,\pi_2 \in \mathcal{A}$ having transformation matrices $A_1,A_2$, then $\pi_1\in[\pi_2]$ if and only if $A_1 \cdot A_2^{-1} \in\BLTA(2,1,\ldots,1)$.  %[\pid]$.
\begin{proof}
This follows dirctly from Lemma~\ref{lem:inv} and the definitions of EC and $[\pid]$. 
\end{proof}
\end{lemma}
%If either one of the two checks fails, the vectors are discarded. 
%The process is repeated until the desired number of automorphisms $M$ is reached.

We can now propose a practical method to list one automorphism for every $\EC$. 
The idea is to start by dividing the affine transformation matrix in $l$ blocks of size $s_1,\ldots,s_l$; a representative for each sub-class of $\EC_i$ will be calculated, independently from the other blocks. 
For each block, all the matrices belonging to $\mathcal{U}(s_i)$ and $\mathcal{P}(s_i)$ are calculated and included as representative of a sub-class, after checking that they do not belong to any already calculated coset through Lemma~\ref{lem:PU_BLT}. 
Next, matrices in the form $UP$, with $U \in \mathcal{U}(s_i)$ and $P \in \mathcal{P}(s_i)$, are included in the list if they pass the check of Lemma~\ref{lem:PU_BLT}. 
When $|\EC_i|$ representatives are found, the searching process stop. 
Next, $\EC$ representatives are calculated by composing block diagonal matrices by mixing among them all the representatives of the $\EC_i$ foun din previous step. 

%from $\mathcal{U}$ and $\mathcal{P}$, that are easy to compute, and mix them to find new cosets. 
%Logic steps:
%\begin{itemize}
%\item every $\mathcal{U}$ and every $\mathcal{P}$ belongs to a different coset (true?)
%\item each coset contains an element from $\mathcal{U} \cdot \mathcal{P}$
%\item there are repetitions, but they can be easily excluded checking group properties
%\end{itemize}
%\comment{It may be good to explain that these steps make sense and they are true.}
%
%
%We now focus on polar codes that follow the UPO and thus have $\BLTA(s)$ as the group of GA automorphisms.  Obviously in this case, $\mathcal{U} \subset \BLTA(s)$ and $\mathcal{P} \subset \BLTA(s)$, and thus the corresponding upper-triangular matrices $U$ have a staircase structure, and the permutation matrices $P$ are block-diagonal with permutation matrices on the diagonal.
%
%Note that $\mathcal{U}$ and $\mathcal{P}$ are easily identified based on the profile $s$ of $\BLTA(s)$.

%\begin{lemma}
%	For a given profile $s$, $(A,b) \in \BLTA(s)$ if and only if it has a PUL decomposition with $P,U,L \in \BLTA(s)$.
%\end{lemma}
%\begin{proof}
%	For the time being, the case $b=0$ and $s=(s_1,s_2)$.
%	
%	First, assume $P,U,L \in \BLTA(s)$, with
%	\begin{align*}
%		P &= \begin{bmatrix} P_1 & 0 \\ 0   & P_4 \end{bmatrix} , &
%		U &= \begin{bmatrix} U_1 & 0 \\ 0   & U_4 \end{bmatrix} , &
%		L &= \begin{bmatrix} L_1 & 0 \\ L_3 & L_4 \end{bmatrix} ,
%	\end{align*}  
%	where $P_1$ and $P_4$ are permutation matrices, $U_1$ and $U_4$ are upper-triangular, $L_1$ and $L_4$ are lower-triangular, and $L_3$ is arbitrary.
%	Note that $P$, $U$ and $L$ necessarily have this structure by their condition.  Then they are a PUL decomposition of $A = PUL$, 
%	\begin{equation*}
%		\begin{bmatrix} A_1 & A_2 \\ A_3 & A_4	\end{bmatrix} 
%		  = \begin{bmatrix} P_1 U_1 & 0 \\ 0   & P_4 U_4 \end{bmatrix} \cdot
%		      \begin{bmatrix} L_1 & 0 \\ L_3 & L_4 \end{bmatrix}  
%		  = \begin{bmatrix} P_1 U_1 L_1 & 0 \\ P_4 U_4 L_3 & P_4 U_4 L_4 \end{bmatrix}  .
%	\end{equation*} 
%	Thus $A \in \BLTA(s)$. 
%	
%	Second, assume that $A \in \BLTA(s)$.  Then by the previous equations, a PUL decomposition with $P,U,L \in \BLTA(s)$ is given by the $P$, $U$, $L$ with 
%	\begin{equation*}
%		L_3 = (P_4 U_4)^{-1} A_3 ,
%	\end{equation*}
%	which exists as $P_4$ and $U_4$ are invertible.
%	
%	For general profiles $s$, the prove follows the same lines; alternatively above prove may be applied recursively.  Finally, for $b \ne 0$, we use the identity $b = PU b_0$, assuming $(L,b_0)$, and notice that $P$ and $U$ are invertible.
%\end{proof}
%
%\begin{theorem}
%	Given $\mathcal{U}$ and $\mathcal{P}$, then 
%	\begin{equation*}
%		\bigl\{ [P U] : P \in \mathcal{P} , U \in \mathcal{U} \bigr\}
%		=  \bigl\{ [A] : A \in \mathcal{A} \bigr\}  ,
%	\end{equation*}
%	i.e., the set of equivalence classes obtained by produces $PU$ is identical to the overall set of equivalence classes in the group of GA automorphisms $\mathcal{A}$.
%\end{theorem}
%\begin{proof}
%	\comment{TBD, but consequence of previous results on BLTL}
%\end{proof}
%Though this holds in general, this theorem has an important practical value for $\BLTA(s)$, as for this case, the sets $\mathcal{U}$ and $\mathcal{P}$ can easily be identified.  According to the theorem, the products $PU$ allow to identify all equivalence classes.  Note, however, that some of the $[PU]$ are identical as the PUL decomposition is not unique.
%
%\comment{The may require refinement, as it was assumed that $\mathcal{L}$ is identical to the SC-absorption group, while it is in general only a subset.}
%
%
%Note that these group properties holds independently of the chosen decoder. 
%In next section, we will focus on classical SC decoding algorithm, analyzing how these properties can be rewritten for this decoder.
%%whether or not $[\pid]$ is equal to $\mathcal{L}$.



